Learning to Learn from Mistakes: Robust Optimization for Adversarial Noise

Sensitivity to adversarial noise hinders deployment of machine learning algorithms in security-critical applications. Although many adversarial defenses have been proposed, robustness to adversarial noise remains an open problem. The most compelling defense, adversarial training, requires a substantial increase in processing time and it has been shown to overfit on the training data. In this paper, we aim to overcome these limitations by training robust models in low data regimes and transfer adversarial knowledge between different models. We train a meta-optimizer which learns to robustly optimize a model using adversarial examples and is able to transfer the knowledge learned to new models, without the need to generate new adversarial examples. Experimental results show the meta-optimizer is consistent across different architectures and data sets, suggesting it is possible to automatically patch adversarial vulnerabilities.

==> acronyms.tex <==
\acrodef{ML}[ML]{Machine Learning}
\acrodef{DL}[DL]{Deep Learning}
\acrodef{DNN}[DNN]{Deep Neural Networks}
\acrodef{SVM}[SVM]{Support Vector Machine}
\acrodef{RL}[RL]{reinforcement learning}




% abbreviations
\acrodef{wrt}[\emph{w.r.t}]{with respect to}
\acrodef{st}[\emph{s.t.}]{such that}


% attacks
\acrodef{fgsm}[FGS]{Fast Gradient Sign}
\acrodef{bim}[BI]{Basic Iterative}
\acrodef{illcm}[ILC]{Iterative Least-likely Class}
\acrodef{jsma}[JSMA]{Jacobian-based Saliency Map Attack}
\acrodef{uap}[UAP]{Universal Adversarial Perturbations}
\acrodef{opa}[OPA]{One Pixel Attack}
\acrodef{pgd}[PGD]{projected gradient descent}
\acrodef{rssa}[RSSA]{Randomised Single Step Attack}
\acrodef{eat}[EAT]{Ensemble Adversarial Training}
\acrodef{gaa}[GAA]{Generative Adversarial Attacks}
\acrodef{gan}[GAN]{Generative Adversarial Networks}
\acrodef{nae}[NAE]{Natural Adversarial Examples}
\acrodef{atn}[ATN]{Adversarial Transformation Networks}
\acrodef{vae}[VAE]{Variational Auto-Encoders}
\acrodef{cfoa}[CFOA]{Complete First Order Adversary}
\acrodef{iid}[i.i.d]{independent and identically distributed}
\acrodef{bpda}[BPDA]{Backward Pass Differentiable Approximation}
\acrodef{alp}[ALP]{Adversarial Logit Pairing}
\acrodef{fbgan}[FB-GAN]{Featurized Bidirectional Generative Adversarial Networks}
\acrodef{sap}[SAP]{Stochastic Activation Pruning}
\acrodef{mat}[MAT]{Multi-strength Adversarial Training}
\acrodef{dam}[DAM]{Dense Associative Memory}
\acrodef{zoo}[ZOO]{Zeroth Order optimisation}
\acrodef{sa}[STA]{Strong Adversary}
\acrodef{lm}[LM]{Linear Models}
\acrodef{dt}[DT]{Decision Trees}
\acrodef{knn}[KNN]{K-nearest Neighbour}




==> content/introduction.tex <==
\section{Introduction}

Premises:
\begin{itemize}
	\item Learning to learn proved more efficient than other optimisers. 
	\item Metalearning helps with sample size - and robust learning needs more samples
	\item In learning2learn the problem is to increase generalisation, which is a huge problem in training robust classifiers (see Madry talk fron NIPS2018)
	\item Related work in HyperNetworks!
	\item There are some phenomenons related to adversarial examples that can benefit from these (?):
		\begin{itemize}
			\item Gradient masking for defences
			\item Obfuscated gradients
			\item Any other gradient related phenomenon (?)
		\end{itemize}
	
	\item Investigate if using a different optimiser affects sensitivity to adversarial examples!
	\item Investigate if using a learned optimiser leads to different decision boundaries
	\item Investigate if we can learn to approximate all perturbations in a set - what if instead of using PGD we can learn an optimiser that finds an approximation of a set and later train with that approximation.
	\item Wald's maxim-min 
	\item Robust Optimization of Unconstrained Binary Quadratic Problems
		\begin{itemize}
			\item In this paper they talk about robust regularization, which is what happens now with DL, although it is not directly named like this. The question is: do we want to achieve regularization? Not really, we would like to design an algorithm that automatically robustly regularizes a function
			\item This was done with least squares, so maybe using this example also helps
			\item 
		\end{itemize}
	\item 
\end{itemize}

The main questions are:
\begin{itemize}
	\item Do other optimizers lead to better decision boundaries?
	\item Can learning an optimizer specially for one task improve the robustness of a model?
	\item 
\end{itemize}
















Notes from literature:
\begin{itemize}
	\item Another popular approach to meta-learning is to interpret the gradient update of SGD as a parametric and learnable function [16] rather than a fixed ad-hoc routine.
	\item To do this? we consider the synaptic learning rule as a parametric function? and we optimize its parameters using standard optimization tools? such as gradient descent ?????
	\item Mostly, these two algorithms must perform the same task: they must leverage the regularities of their respective problems in order to efficiently solve them. However, there are differences in the time scale and scope of their problems. The supervisory process has a broader scope. It must ignore the details unique to .specific problems, and look for symmetries over a long time scale, while the opposite is true for a subordinate learning scheme.
	\item 

\end{itemize}




Use the capacity of the learning rule to describe adaptability in robust environments.
